Formality is Favored: Unraveling the Learning Preferences of Large Language Models on Data with Conflicting Knowledge

Having been trained on massive pretraining data, large language models have shown excellent performance on many knowledge-intensive tasks. However, pretraining data tends to contain misleading and even conflicting information, and it is intriguing to understand how LLMs handle these noisy data during training. In this study, we systematically analyze LLMs' learning preferences for data with conflicting knowledge. We find that pretrained LLMs establish learning preferences similar to humans, i.e., preferences towards formal texts and texts with fewer spelling errors, resulting in faster learning and more favorable treatment of knowledge in data with such features when facing conflicts. This finding is generalizable across models and languages and is more evident in larger models. An in-depth analysis reveals that LLMs tend to trust data with features that signify consistency with the majority of data, and it is possible to instill new preferences and erase old ones by manipulating the degree of consistency with the majority data.

==> tmp/TODO.tex <==
1. 信源混合训练 -> 更低方差的可视化 *
2. 图表,
3. Setup 简洁， 统一描述
4. Section 找一些社科文献
5. pythia-13b 的实验 *
6. 地理三层级 * 

1. 多语言多模型（4模型 * 3实验）
1 * 3
2. 4种风格单独训练，statement准确率变化
7 * 1

==> tmp/note.tex <==
1. style: 4 style, 6 PR
2. grammar: 1 PR 
3. conflict knowledge: 1 PR

PR > 50
8 PR, 6 field


5/6 information field, 

TODO
